Sorting and Transforming Program Repair Ingredients via Deep Learning Code Similarities

In the field of automated program repair, the redundancy assumption claims large programs contain the seeds of their own repair. However, most redundancy-based program repair techniques do not reason about the repair ingredients---the code that is reused to craft a patch. We aim to reason about the repair ingredients by using code similarities to prioritize and transform statements in a codebase for patch generation. Our approach, DeepRepair, relies on deep learning to reason about code similarities. Code fragments at well-defined levels of granularity in a codebase can be sorted according to their similarity to suspicious elements (i.e., code elements that contain suspicious statements) and statements can be transformed by mapping out-of-scope identifiers to similar identifiers in scope. We examined these new search strategies for patch generation with respect to effectiveness from the viewpoint of a software maintainer. Our comparative experiments were executed on six open-source Java projects including 374 buggy program revisions and consisted of 19,949 trials spanning 2,616 days of computation time. DeepRepair's search strategy using code similarities generally found compilable ingredients faster than the baseline, jGenProg, but this improvement neither yielded test-adequate patches in fewer attempts (on average) nor found significantly more patches than the baseline. Although the patch counts were not statistically different, there were notable differences between the nature of DeepRepair patches and baseline patches. The results demonstrate that our learning-based approach finds patches that cannot be found by existing redundancy-based repair techniques.

==> bak/authors.tex <==
\author{Martin~White,~Michele~Tufano}
\affiliation{%
  \institution{College~of~William~\&~Mary}
  \streetaddress{P.O.~Box~8795}
  \city{Williamsburg}
  \state{Virginia}
  \postcode{23187--8795}
}
\email{{mgwhite, mtufano}@cs.wm.edu}

%\author{Michele~Tufano}
%\affiliation{%
%  \institution{College~of~William~\&~Mary}
%  \streetaddress{P.O.~Box~8795}
%  \city{Williamsburg}
%  \state{Virginia}
%  \postcode{23187--8795}
%}
%\email{mtufano@cs.wm.edu}

\author{Mat{\'i}as~Mart{\'i}nez}
\affiliation{%
  \institution{University~of~Valenciennes}
  \streetaddress{\ed{59313~Valenciennes~Cedex~9}}
  \city{\ed{Valenciennes}}
  \country{France}
}
\email{matias.martinez@univ-valenciennes.fr}

\author{Martin~Monperrus}
\affiliation{%
  \institution{KTH~Royal~Institute~of~Technology}
  \streetaddress{\td}
  \city{Stockholm}
  \country{Sweden}
}
\email{martin.monperrus@csc.kth.se}

\author{Denys~Poshyvanyk}
\affiliation{%
  \institution{College~of~William~\&~Mary}
  \streetaddress{P.O.~Box~8795}
  \city{Williamsburg}
  \state{Virginia}
  \postcode{23187--8795}
}
\email{denys@cs.wm.edu}

% The default list of authors is too long for headers}
\renewcommand{\shortauthors}{M.~White~et~al.}

==> bak/keywords.tex <==
\keywords{
automated~program~repair,~%
deep~learning,~%
%manifold~learning,~%
neural~networks%,~%
%%code~clone~detection,~%
%code clones,~%
%language~models,~%
%simulated~annealing
}

==> bak/validation.tex <==
\section{Empirical~Validation}
\label{sec:validation}

We now evaluate DeepRepair with the following research questions:~%
\begin{description}
\item[\emph{RQ1}]
Do code similarities based on deep learning improve fix space navigation as compared to a uniform random search strategy?
\item[\emph{RQ2}]
Does variable resolution based on deep learning effectively transform repair ingredients as compared to {a default variable resolution algorithm that does not transform ingredients?}~%
\item[\emph{RQ3}]
Does DeepRepair, our learning-based approach that uses code similarities and transforms repair ingredients, improve fix space navigation as compared to the default jGenProg~\cite{Martinez:2016} engine?~%
\item[\emph{RQ4}]
Does DeepRepair generate higher quality patches than the default jGenProg engine?~%
%\matias{It would be interesting to analyze the quality of patches found to know whether using clone ingredients produce ``better'' patches than using other strategies. In our previous experiments, we manually analyzed the patches generated by Astor for determining their correctness, readability, etc.}
%\denys{I think the fact that we are learning in the same space can help us create not only correct, but also readable patches?}
%\marty{Example from prior work: Are the generated patches correct, beyond passing the test suite?}
%\marty{THINKING: [Quality] How complete (i.e., coverage of important information) are the patches generated? [Quality] How concise (i.e., level of redundant information) are the patches generated? [Usefulness] How well can the patches help developers in fixing bugs?}
\end{description}
% * <martingwhite@gmail.com> 2016-09-05T23:25:09.701Z:
%
% Any recommended changes to the research questions or are there other research questions to consider?
%
% ^ <martin.monperrus@univ-lille1.fr> 2016-09-09T13:18:57.541Z:
%
% slightly modified RQ1 and RQ2
%
% ^.
% * <martingwhite@gmail.com> 2016-09-07T00:40:03.713Z:
% 
% For RQ4, aimed at judging the quality of patches, are there any other empirical studies that would be good to review aside from "Automatic Repair of Real Bugs: An Experience Report on the Defects4J Dataset"?
% 
% ^ <martin.monperrus@univ-lille1.fr> 2016-09-09T13:19:38.564Z:
%
% There are very few such deep analysis.
%
% ^.
\begin{comment}
\ed{In order to find a patch, a search strategy must find ingredients that can be applied at the modification points in the program variants.}~%
\ed{Consequently, the ingredient must ``fit'' in the sense that all variable accesses must be in scope, i.e., the ingredient must \emph{satisfy} the context of the modification point such that the name and type of each variable access in the ingredient must correspond to a variable in the context.}~%
\ed{We refer to these ingredients as \emph{satisfiable} ingredients.}~%
\ed{In their study, measuring the graftability of changes to a codebase, Barr et al.~\cite{Barr:2014} only consider line-granular snippets that match exactly (ignoring whitespace).}~%
\ed{However, snippets in a codebase are valuable clues on how to generate or synthesize meaningful code fragments, so our intent with using embeddings is to transform otherwise unsatisfiable ingredients.}~%
\ed{With the ability to transform ingredients, our generate-and-validate approach can use the syntax in a candidate ingredient and adapt its contents for a particular context.}~%
\ed{Applying a satisfiable ingredient may or may not improve a program variant's fitness, but strategies that can consistently find satisfiable ingredients may be able to focus their search in areas of the complex search space where fixes are likely to exist}.~%
\end{comment}

%\input{tab/projects}

%\subsection{Scope~of~the~Experiment}
The goal of our empirical study {was} to \textbf{analyze} %the effectiveness of different 
ingredient search strategies for the \textbf{purpose} of evaluation with \textbf{respect} to %\ed{their} 
effectiveness~\cite{Wohlin:2000}.~%
Our empirical study was from the \textbf{point~of~view} of the software maintainer in the \textbf{context} of {six} open-source Java projects, a collection of (real) reproducible bugs, and a collection of JUnit test cases~\cite{Wohlin:2000}.~%
The baseline configuration was the (uniform) random search strategy where ingredients were selected from a pool of equiprobable statements.~%
We configured the baseline with a cache so the same modification instance (i.e., ingredient and operator instance) were never \ed{attempted} more than once to improve its efficiency.~%
The baseline was also configured with a default variable resolution algorithm that analyzed the variable accesses in a repair ingredient, matching accesses' names and types to variables in scope.~%
If at least one access failed to match a variable in scope, then the ingredient was discarded.~%
% * <martingwhite@gmail.com> 2016-09-05T23:25:56.993Z:
%
% Any recommended changes to the experimental definition?
%
% ^ <martin.monperrus@univ-lille1.fr> 2016-09-09T13:21:52.292Z:
%
% Sentence quite long. I would split in several parts, or if we want a direct relation to Wohin, let's do a description list
%
% ^.
%\subsection{Context~Selection}
%\subsection{Hypothesis~Formulation}


We formalize our experiment into the following hypotheses:~%
\begin{description}
\item[$H_0^{1a}$]
%The {similar fragment search strategy} generates the same number of test-adequate patches (on average) as the baseline.~%
Using code similarities generates the same number of test-adequate patches (on average) as the baseline.~%
\item[$H_0^{1b}$]
%The {similar search strategy} attempts\footnote{An \emph{attempt} is defined to be a request sent to the fix space for an ingredient.} the same number of ingredients %(on average)
%before finding a {test-adequate patch} as the baseline.~%
Using code similarities attempts\footnote{An \emph{attempt} is defined to be a request sent to the fix space for an ingredient.} the same number of ingredients before finding a {test-adequate patch} as the baseline.~%
\item[$H_0^{2a}$]
Variable resolution using embeddings generates the same number of test-adequate patches %(on average)
as the baseline.~%
\item[$H_0^{2b}$]
%Variable resolution using word embeddings rejects on average the same number of ingredients before finding a \ed{satisfiable} ingredient as the variable resolver without word embeddings.~%
Variable resolution using embeddings attempts the same number of ingredients %(on average)
before finding a {test-adequate patch} as the baseline.~%
\item[$H_0^{3a}$]
%The {similar search strategy with the embeddings-based variable resolution algorithm} generates the same number of {test-adequate patches} as the baseline.~%
DeepRepair generates the same number of {test-adequate patches} as the baseline.~%
\item[$H_0^{3b}$]
%The {similar search strategy with the embeddings-based variable resolution algorithm} attempts the same number of ingredients %(on average)
%before finding a {test-adequate patch} as the baseline.~%
DeepRepair attempts the same number of ingredients before finding a {test-adequate patch} as the baseline.~%
\item[$H_0^4$]
{There is no significant difference in quality (i.e., correctness) between patches generated by DeepRepair and the default jGenProg engine.}~%
\end{description}
% * <martingwhite@gmail.com> 2016-09-05T23:27:01.618Z:
%
% Any recommended changes to the hypotheses or are there new hypotheses to consider?
%
% ^.
%\subsection{Variables~Selection}
We chose the following \textbf{dependent~variables}:~number of test-adequate patches and
number of ingredients attempted.~%before finding a valid ingredient and time to repair.
We chose the following \textbf{independent~variables} (emphasizing the factors):~%\emph{repair~engine} (JGenProg, JKali, JMutRepair),
\emph{ingredient~search~strategy}, \emph{scope}, \emph{clone granularity}, \emph{variable resolution algorithm}, fault localization threshold, maximum number of suspicious candidates, and programming language.~%
% * <martingwhite@gmail.com> 2016-09-05T23:29:49.086Z:
%
% Is anything missing from this list of independent variables? There are many variables that need to be set for a given run...I have a long list...but don’t believe many of them need to be declared.
%
% ^.
% * <martingwhite@gmail.com> 2016-09-05T23:31:11.657Z:
%
% @Matias agrees that \emph{repair engine} (JGenProg, JKali, and JMutRepair) can be removed from consideration, and that it should be enough to simply use the JGenProg engine and compare its typical random strategy to our clone strategy for the paper's evaluation.
%
% ^.
% * <martingwhite@gmail.com> 2016-09-05T23:31:49.287Z:
%
% Note that Defects4J attributes (e.g., ProjectID and RevisionID) are not included as variables; these attributes will be used to define the experimental units.
%
% ^.
% * <martingwhite@gmail.com> 2016-09-05T23:33:01.769Z:
%
% However, one important discussion point is how we handle training. It seems that we will have to train on each <ProjectID, BuggyID> and evaluate on the corresponding <ProjectID, FixedID>. That’s a lot of training for the evaluation but the fact that Defects4J does not give us enough information to reliably sequence the buggy revisions means there’s no way to reliably reuse models.
%
% ^.
% * <martingwhite@gmail.com> 2016-09-05T23:33:47.980Z:
%
% Incidentally, I don’t want to take the focus away from refining this validation specification, but this problem of what do we train on was what prompted the questions in the Astor email thread on the vocabulary differences between buggy and fixed revisions.
%
% ^.
% * <martingwhite@gmail.com> 2016-09-05T23:35:33.597Z:
%
% My key concern with the dependent and independent variables is I don’t want to complicate the analysis with multiple hypotheses, more than two factors, and/or more than two treatments if it’s not necessary.
%
% ^.
The fault localization threshold was fixed at 0.1;~%
% * <martingwhite@gmail.com> 2016-09-05T23:37:56.793Z:
%
% Is there (technical) justification for why we typically use 0.1?
%
% ^ <martin.monperrus@univ-lille1.fr> 2016-09-09T13:23:56.488Z:
%
% Not really, however this should not have any impact or experiment besides raw performance (in seconds), because it's rather orthogonal to what we look at/
%
% ^.
the maximum number of suspicious candidates was fixed at 1,000;~%
% * <martingwhite@gmail.com> 2016-09-06T00:43:23.537Z:
%
% Is there (technical) justification for why we typically use 1,000?
%
% ^ <martin.monperrus@univ-lille1.fr> 2016-09-09T13:24:16.346Z:
%
% It's simply an upper bound on the computational budget
%
% ^.
and the language was fixed on Java.~%
The random seed for each experimental configuration ranged from one to {three}.~%
%\matias{It could be added the fault localization formula used in the experiment. Astor uses Ochiai formula encoded in GZoltar tool, but both formula and tool could be replaced.}
%\ed{For our qualitative study, analyzing patch correctness, we} \td

%\subsection{Selection~of~Subjects}

%\subsection{Experiment~Design}
% * <martingwhite@gmail.com> 2016-09-06T00:49:17.839Z:
%
% Here is the design for $H_0^1$...There will be slight differences depending on the hypothesis. What is the most efficient way to organize/consolidate the designs?
%
% ^.
We designed comparative experiments to measure the statistical significance of our results.~%
Typically, empirical studies in the field report the number of test-adequate patches found, but we conducted a large-scale study, report the number of test-adequate patches found, and measure the statistical significance of differences to contextualize the results.~%
{For our quantitative study,} the treatments in our experimental design were the ingredient search strategies.~%
% * <martingwhite@gmail.com> 2016-09-06T00:45:14.922Z:
%
% Ingredient search strategies is a factorial of scope (local, package, global) and clone granularity (method, class); random serves as the control.
%
% ^.
The experimental units were the buggy program revisions, and the responses were the number of test-adequate patches found and the number of ingredients attempted before finding a {test-adequate patch}.~%
% * <martingwhite@gmail.com> 2016-09-06T00:47:46.939Z:
% 
% One design detail that is still missing is how we apply treatments to units...Should we randomly assign treatments to <ProjectID, BuggyID> or apply each treatment to every <ProjectID, BuggyID>?
% 
% ^.
%\ed{For our qualitative study,} \td
%\subsection{Instrumentation}
%\subsection{Validity~Evaluation}
%\xx
We %discuss limitations of our empirical study in Sec.~\td and
consolidate threats to the validity of our work in Sec.~\ref{sec:threats}.~%

%\input{tab/patches}
%\input{fig/patch_attempts}

\subsection{Data~Collection~Procedure}

The first stage of our recognition phase involved creating a model of source code (Sec.~\ref{sub:recognition}).~%
We used Spoon~\cite{Pawlak:2015}, an open-source library for analyzing and transforming Java source code, to build a model for each buggy program revision.~%
Given the source code models, we implemented program processors for querying program elements at three levels:~file-, type-, and executable-level granularity.~%
Types included classes and interfaces, and executables included methods and constructors, but we omitted anonymous blocks.~%
We only queried top-level types and executables to control the number of similarities to be computed.~%
In this context, by ``top-level,'' we mean types or executables that did not have a parent type or executable, respectively.~%
For example, a nested class would not be included, but its enclosing class may be included.~%
%Then we extracted the string of lexical elements for each program element along with its corresponding key to build three corpora.~%
Then we extracted the yield~\cite{Aho:2006} from each element's {syntax} tree along with its corresponding key to build three corpora.~%
So each line of a type-level corpus corresponded to a class or interface in the program.~%
The only normalization we performed was replacing character, float, integer, and string literal values %in the file-level corpora 
with their respective type.~%

%\input{fig/ing_attempts}

The first stage of our learning phase involved inducing neural network language models from the normalized file-level corpora (Sec.~\ref{sub:learning}).~%
We used word2vec~\cite{Mikolov:2013:ICLR,Mikolov:2013:NIPS,Mikolov:2013} to learn embeddings for \emph{each} buggy program revision from the corresponding file-level corpus.~%
The reason we selected word2vec over other architectures is because the models can be trained quickly, and we only used the language models' embeddings to initialize the embeddings for the recursive autoencoders rather than randomly initialize them.~%
%A skip-gram predicts the context words given a word~\cite{Rong:2014}.~%
We used the skip-gram model and set the size of the word vectors to 400 in accordance with previous studies using similar subject systems~\cite{White:2016}.~%
We set the maximum skip length between words to 10, used a hierarchical softmax to optimize the computation of output vectors' updates~\cite{Rong:2014}, and trained each model for 20 iterations.~%
The language models enabled us to transform the file-level corpus for each program revision into streams of embeddings.~%
Then we trained recursive autoencoders to encode these streams of embeddings.~%
The encoders used hyperbolic tangent activation functions (i.e., $f\defeqq\text{tanh}$ in Eq.~\eqref{eq:z}), used L-BFGS~\cite{Nocedal:1980} to optimize costs in batch mode, and trained for up to 50 epochs.~%
After an encoder was trained on a revision's file-level corpus, we used it to encode every type and executable in the revision's type- and executable-level corpora, respectively.~%
Given the encodings, we computed the pairwise Euclidean distance between each pair of types in the type-level corpus and each pair of executables in the executable-level corpus to measure similarities for each program revision.~%
We also extracted the term embeddings from the trained encoder and clustered them using $k$-means.~%
For each revision, to determine $k$, we used simulated annealing, initializing both $k$ and the temperature to be the square root of the corresponding vocabulary size.~%
The reason we chose the square root of the vocabulary size is because of its effectiveness in related contexts that categorize words~\cite{Mikolov:2011:RNNLM}.~%
The objective we optimized was minimizing the number of points with negative silhouette values.~%
At the end of the learning phase, each buggy revision had a cached list of executable- and type-level similarities as well as a categorization for identifiers.~%

The final phase of our technical approach involved automatically repairing buggy program revisions (Sec.~\ref{sub:repair}).~%
To run program repair experiments, we used Astor~\cite{Martinez:2016:ASTOR}, an automatic software repair framework for Java.~%
%Our subject systems included five open-source Java projects (Tab.~\ref{tab:projects}).
%We used ANTLR~4 to generate a lexical analyzer for Java and tokenize the buggy and fixed program revisions for each bug and every project in the Defects4J database version 1.0.1~\cite{Just:2014,Just:2014:ISSTA}.
%Our lexical analyzer replaced literal values with their corresponding literal type.
%Then, for each project, we replaced hapax legamenon with \texttt{<unk>} to build open vocabulary projects~\cite{Jurafsky:2009}.
Our subject systems comprised {six} open-source Java projects including {374} buggy program revisions in Defects4J database version {1.1.0}~\cite{Just:2014,Just:2014:ISSTA}.\footnote{We could not build the Spoon model for Mockito bugs 1--21, which was likely because of missing or incompatible dependencies.}~%
In Tab.~\ref{tab:projects}, we report median values since each project has several buggy program revisions.~%
{Within the Astor framework, we leveraged GZoltar~\cite{Campos:2012}, a spectrum-based fault localization tool, to compute the Ochiai formula~\cite{Abreu:2006} for statements' suspicious values.}~%
%\td
Each trial corresponded to a seeded treatment, which was a factorial of strategy and scope.~%
Empirical studies indicate that fragment locality matters in software maintenance and evolution, so we analyzed three different levels of scope:~local, package, and global~\cite{Martinez:2014}.~%
{For local scope, Astor builds the ingredient search space by amalgamating the distinct set of classes that contain at least one suspicious statement.}~%
{For package scope, Astor computes the distinct set of packages that contain at least one suspicious statement and builds the ingredient search space using the set of classes in those packages.}~%
{For global scope, Astor builds the ingredient space using all classes from the application under repair.}~%
In total, we ran {20,196} trials ({374} buggy program revisions $\times$ 18 configurations $\times$ {3} random seeds) on subclusters comprising 64 compute nodes running Red Hat Enterprise Linux~6.2.~%, in the SciClone computing complex.~%
Each compute node was a Dell PowerEdge C6100 serving two Intel Xeon~X5672 quad-core processors at 3.2~GHz with 12~MB L3~cache and at least 48~GB of 1333~MHz main memory.~%
Each trial was allocated {two} (hyper-threaded) cores and %, at least {11}~GB of main memory, and %ran for at most three hours.~%
evolved one program variant for three hours using three repair operators:~InsertAfterOp, InsertBeforeOp, and ReplaceOp.~%
\emph{We did not include RemoveOp in our operator space because we only focused on repair operators that reuse code}.~%
%\marty{THINKING: Under-specified bugs}
We also wanted to guard against meaningless patches that simply remove functionality.~%
%\ed{Moreover, previous studies reported\dots}

\input{tab/projects}

\subsection{Analysis~Procedure}

%\subsubsection{RQ1}
%\noindent\textbf{RQ1.}~
\subsubsection*{RQ1}~We analyzed the effectiveness of fix space navigation strategies in two parts.~%
The {first} part analyzed strategies' effectiveness at generating test-adequate patches.~%
We used the non-parametric Wilcoxon test with a Bonferroni correction to compare the number of test-adequate patches using the baseline strategy versus the similar fragment search strategy at executable- and type-level granularity.~%
{To complement our statistical analysis on number of test-adequate patches found, we also computed the difference between the set of baseline patches and the set of DeepRepair patches.}~%
Specifically, if $D$ is the set of DeepRepair patches, and $B$ is the set of baseline patches, then we compute and report $\left\vert{D\setminus B}\right\vert/\left\vert{D}\right\vert$, the percentage of DeepRepair patches that were not found by the baseline.~%
The {second} part analyzed the number of attempts to generate test-adequate patches.~%
We used the non-parametric Mann-Whitney test with a Bonferroni correction to compare the number of attempts to generate test-adequate patches using the baseline configuration and the similar fragment search strategy at executable- and type-level granularity.~%
To complement our analysis on number of attempts, we also plotted the number of attempts to generate {compilable} ingredients.~% for each level of scope and every strategy.~%

%\subsubsection{RQ2}
%\noindent\textbf{RQ2.}~
\subsubsection*{RQ2}~We analyzed effectiveness in two parts.~%
We used the Wilcoxon test to compare the number of test-adequate patches using the baseline strategy versus the uniform random search strategy with the embeddings-based variable resolution algorithm.~%
{The algorithm gives the baseline configuration the ability to transform repair ingredients containing variable accesses that are out of scope.}~%
{We also computed the difference between the set of baseline patches and the set of DeepRepair patches.}~%
Additionally, we used the Mann-Whitney test to compare the number of attempts to generate test-adequate patches and plotted the number of attempts to generate compilable ingredients.~%

%\subsubsection{RQ3}
%\noindent\textbf{RQ3.}~
\subsubsection*{RQ3}~Our experimental design for \emph{RQ3} was virtually identical to our design for \emph{RQ1} except here we compared the baseline configuration to the similar fragment search strategy with the embeddings-based variable resolution algorithm.~%

%\subsubsection{RQ4}
%\noindent\textbf{RQ4.}~
\subsubsection*{RQ4}~We used correctness as a proxy for quality.~%
We manually examined a random sample of generated patches to assess correctness.~%
Martinez et al.~\cite{Martinez:2015} defined the \emph{correctness} of a patch to be one of three values:~correct, incorrect, or unknown.~%
\emph{Correct} denotes a patch is equivalent (according to the judge's understanding) to the human-written patch.~%
Judges were also prompted for their confidence in their correctness rating where confidence was one of four values:~high, moderate, slight, and none.~%
Additionally, for reproducibility, we assessed the readability of each patch, where the \emph{readability} of a patch was either easy, medium, or hard in accordance with previous studies on patch correctness~\cite{Qi:2015,Martinez:2016}.~%
We define readability to be the subjective qualification of how easily the patch can be understood.~%
Readability is a subjective aggregation of different quantitative metrics: patch size in number of lines, number of involved variables, number of method calls, and the types of AST elements being inserted or replaced.~%
There is no accepted quantitative aggregation of these metrics, and we think that a quantitative aggregation would be project- and even bug-dependent.~%
In addition to the random sample, we also evaluated the patches generated by the baseline that were not found by DeepRepair and patches generated by DeepRepair that were not found by the baseline.~%


\michele{More details on the sampling process: 5 bugs were randomly selected from the 3 projects containing patches. For each bug, we first randomly select a scope, then randomly a baseline patch and a DeepRepair patch. In total 3 judges have to evaluate 30 patches. In the second round of evaluation the judges discussed the results in order to achieve three-judges agreement on the patch correctness.}

==> ccs.tex <==
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010257.10010293.10010294</concept_id>
<concept_desc>Computing methodologies~Neural networks</concept_desc>
<concept_significance>500</concept_significance>
</concept>
\begin{comment}
<concept>
<concept_id>10010147.10010178.10010205.10010209</concept_id>
<concept_desc>Computing methodologies~Randomized search</concept_desc>
<concept_significance>100</concept_significance>
</concept>
<concept>
<concept_id>10011007.10011006.10011073</concept_id>
<concept_desc>Software and its engineering~Software maintenance tools</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10011007.10011074.10011099.10011102.10011103</concept_id>
<concept_desc>Software and its engineering~Software testing and debugging</concept_desc>
<concept_significance>500</concept_significance>
</concept>
\end{comment}
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Neural networks}
%\ccsdesc[100]{Computing methodologies~Randomized search}
%\ccsdesc[300]{Software and its engineering~Software maintenance tools}
%\ccsdesc[500]{Software and its engineering~Software testing and debugging}

==> fig/approach.tex <==
\begin{figure}[t]
\missingfigure[figcolor=white]{Approach}
\centering
\caption{\td}
\label{fig:approach}
\end{figure}

==> fig/chart.tex <==
\begin{figure}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}[node distance=1.5cm,auto,every node/.style={outer sep=0}] %node distance=2cm
\tikzstyle{decision}=[diamond,draw,text width=4em,text badly centered,node distance=2cm,inner sep=0pt] %text width=4.5em, node distance=3cm
\tikzstyle{block}=[rectangle,draw,text width=5em,text centered,rounded corners,minimum height=1em] %minimum height=4em
\tikzstyle{line}=[draw,-latex']
\tikzstyle{cloud}=[draw,ellipse,node distance=2.5cm,minimum height=1em] %node distance=3cm
\node [block,fill=gray!50] (lexical) {\small\sc lexical};
\node [cloud,left of=lexical] (system) {\small\sc system};
\node [block,right of=lexical,node distance=2.5cm,fill=gray!50] (syntactic) {\small\sc syntactic}; %node distance=3cm
\node [decision,below of=syntactic] (decide) {\small\sc combine method};
\node [block,left of=decide,node distance=2.5cm,fill=red] (RtNN) {\small\sc R{t}NN};
\node [block,below of=decide,node distance=2cm,fill=red] (RvNN) {\small\sc R{v}NN}; %node distance=3cm
\node [block,right of=RvNN,node distance=2.5cm] (ast2bin) {\small\sc ast2bin}; %node distance=3cm
\node [cloud,left of=RvNN] (embeddings) {\small\sc embeddings};
\node [block,below of=RvNN] (match) {\small\sc match};
\node [cloud,right of=match] (clones) {\small\sc clones};
\path [line] (lexical) -- node (temp0) {} (RtNN);
\path [line] (lexical) -- (syntactic);
\path [line] (syntactic) -- node (temp1) {} (decide);
\path [line] (decide) -- node {\small\sc greedy} (RvNN);
\path [line] (decide) -| node [near start] {\small\sc ast-based} (ast2bin);
\path [line] (RvNN) -- (match);
\path [line] (ast2bin) -- (RvNN);
\path [line] (system) -- (lexical); %,dashed
\path [line] (RtNN) -- (embeddings); %,dashed
\path [line] (embeddings) -- (RvNN); %,dashed
\path [line] (match) -- (clones); %,dashed
\end{tikzpicture}
}
\caption{\td}
\label{fig:chart}
\end{figure}

==> fig/repair.tex <==
\begin{figure*}
\centering
\begin{subfigure}[b]{0.4\textwidth}
\centering
\input{lst/suspicious.tex}
\caption{\td}
\label{fig:suspicious}
\end{subfigure}\hfill
%add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. (or a blank line to force the subfigure onto a new line)
\begin{subfigure}[b]{0.6\textwidth}
\centering
\input{lst/simlist.tex}
\caption{\td}
\label{fig:simlist}
\end{subfigure}
\caption{\td}
\label{fig:repair}
\end{figure*}

==> fig/tsne.tex <==
\begin{figure}[t]
\centering
%\missingfigure[figcolor=white]{t-SNE}
%\includegraphics[width=0.99\columnwidth]{tsne}
\includegraphics[trim={15cm 0 0 0},clip,width=0.99\columnwidth]{tsne}
\vspace{-0.5\baselineskip}
\caption{Math-63 identifiers' embeddings (best viewed in color) where positions have been jittered to avoid overplotting and colors correspond to clusters.}
\vspace{-1.5\baselineskip}
\label{fig:tsne}
\end{figure}

==> lst/simlist.tex <==
\begin{lstlisting}[caption={\td},label={lst:simlist},numbers=left]
public double solve(final UnivariateRealFunction, double, double)
public static double[] bracket(UnivariateRealFunction, double, double, double, int)
public static double midpoint(double, double)
public double solve(final UnivariateRealFunction, double, double, double)
public double solve(double, double, double)
public static double[] bracket(UnivariateRealFunction, double, double, double)
public BisectionSolver()
private static void setup(UnivariateRealFunction)
public BisectionSolver(UnivariateRealFunction)
\end{lstlisting}
\begin{comment}
public double solve(double min, double max)
private UnivariateRealSolverUtils()
public static double solve(UnivariateRealFunction, double, double)
public static double solve(UnivariateRealFunction, double, double, double)
\end{comment}

==> lst/suspicious.tex <==
\begin{lstlisting}[caption={\td},label={lst:suspicious},mathescape=true,numbers=left]
B72  1.0 return solve(min, max);
B66  0.7 return solve(f, min, max);
B79  0.5 clearResult();
B80  0.5 verifyInterval(min, max);
B85  0.5 int i = 0;
B86  0.5 while (i < maximalIterationCount) {...}
B87  0.5 m = UnivariateRealSolverUtils.midpoint(min, max);
B88  0.5 fmin = f.value(min);
U223 0.3 return (a + b) * .5;
\end{lstlisting}

==> scr/IEEE.abstract.tex <==
\IEEEtitleabstractindextext{%
\begin{abstract}
%Background: Give a brief introducing notice about the motivation for conducting the study. Example: ``Software developers have a plethora of development technologies from which to choose, but often little guidance for making the decision.''
In the field of automated program repair, the {redundancy assumption} %is an empirically validated assumption that %presumes
claims large programs contain the seeds of their own repair.~%
However, most redundancy-based program repair techniques do not reason about the repair ingredients---the code that is reused to craft a patch.~%
%\xx
%Objective: Describe the aim of the study, including the object under examination, the focus, and the perspective. Example: ``We examined <technique1> vs. <technique2> with regard to fault detection rates from the viewpoint of a quality engineer.''
We aim to reason about %the code %that is reused
the repair ingredients by using code similarities to prioritize and transform statements in a codebase for patch generation.~%
Our approach, DeepRepair, relies on deep learning to reason about code similarities.~%the similarity of code.~%elements.~%(e.g., classes, methods, and identifiers) \xx
%such that
Code fragments at well-defined levels of granularity in a codebase can be sorted according to their similarity to suspicious elements (i.e., code elements that contain suspicious statements) and statements can be transformed by mapping out-of-scope identifiers to similar identifiers in scope.~%
We examined these new search strategies for patch generation with respect to effectiveness from the viewpoint of a software maintainer.~%
%Method: Describe which research method was used to examine the object (e.g., experimental design, number and kind of participants, selection criteria, data collection and analysis procedures).
%Example: ``We conducted a controlled experiment using a 2x2 factorial design with 24 randomly assigned undergraduate students participating. The data were collected with the help of questionnaires and analyzed using ANOVA.''
Our comparative experiments were executed on six open-source Java projects including 374 buggy program revisions and consisted of {19,949} trials spanning {2,616} days of computation time.~%
%\xx
%Results: Describe the main findings. Example: ``<technique1> was significantly more %effective than <technique2> at an alpha level of 0.05.''
%DeepRepair's search strategy using code similarities generally found compilable ingredients faster than the baseline, but this {improvement} neither yielded test-adequate patches in fewer attempts (on average) nor found significantly more patches than the baseline.~%
DeepRepair's search strategy using code similarities generally found compilable ingredients faster than the baseline, jGenProg, but this {improvement} neither yielded test-adequate patches in fewer attempts (on average) nor found significantly more patches than the baseline.~%
Although the patch counts were not {statistically} different, there were notable differences between the nature of DeepRepair patches and baseline patches.~%
%Limitations: Describe the major limitations of the research, if any. Example: ``Generalization of results is limited since the analyzed technique was applied only to specify systems smaller than 10.000 lines of code.''
%\td
%Conclusion: Describe the impact of the results. Example: ``The result reinforced existing evidence regarding the superiority of <technique1> over <technique2>.'' Furthermore, to address practitioners’ information need regarding cost, benefits, risks, and transition issues shall be described.
%The results demonstrate that our learning-based approach to reasoning about the code that is reused using similarities finds patches that cannot be found by traditional generate-and-validate techniques.~%
%The results demonstrate that our learning-based approach finds patches that cannot be found by traditional generate-and-validate techniques and hence is complementary to existing approaches.~%
The results demonstrate that our learning-based approach finds patches that cannot be found by existing redundancy-based repair techniques.~% and hence is complementary to existing approaches.~%, thereby complementing existing approaches.~%
%The recommendation to include the element Limitations follows a suggestion made in XXX, since every piece of evidence has its limitations. This additional information will help readers judge transferability of the results to their own context. It will also help to prevent uncritical acceptance by the reader XXX.
%Some publishers limit the length of the abstract by number of words or number of lines. In this case we suggest prioritizing the traditional elements: background (one sentence), objective, method, results, and conclusion and to omit the structuring words by keeping the structure.
\end{abstract}
\begin{IEEEkeywords}
Automated~program~repair,~%
deep~learning,~%
%manifold~learning,~%
neural~networks,~%
%code~clone~detection,~%
code~clones,~%
language~models,~%
simulated~annealing
\end{IEEEkeywords}}

==> scr/IEEE.authors.tex <==
\author{
\IEEEauthorblockN{
Martin~White\IEEEauthorrefmark{1},
Michele~Tufano\IEEEauthorrefmark{1},
Mat{\'i}as~Mart{\'i}nez\IEEEauthorrefmark{2}, 
Martin~Monperrus\IEEEauthorrefmark{3}, and
Denys~Poshyvanyk\IEEEauthorrefmark{1}}
\IEEEauthorblockA{
\IEEEauthorrefmark{1}%Department~of~Computer~Science\\
College~of~William~and~Mary,~Williamsburg,~Virginia~23187--8795\\
Email:~\{mgwhite,~mtufano,~denys\}@cs.wm.edu}
\IEEEauthorblockA{
\IEEEauthorrefmark{2}%\td\\
University~of~Valenciennes,~Malvache~Building,~Campus~Mont~Houy,~59313~Valenciennes~Cedex~9\\
Email:~matias.martinez@univ-valenciennes.fr}
\IEEEauthorblockA{
\IEEEauthorrefmark{3}%\td\\
University~of~Lille~and~INRIA,~Cite~Scientifique,~59655~Villeneuve~d'Ascq~Cedex\\
Email:~martin.monperrus@univ-lille1.fr}
}
\begin{comment}
\author{
\IEEEauthorblockN{Martin~White}
\IEEEauthorblockA{
Department~of~Computer~Science\\
College~of~William~and~Mary\\
Williamsburg,~Virginia~23187--8795\\
Email:~mgwhite@cs.wm.edu}
\and
\IEEEauthorblockN{Michele~Tufano}
\IEEEauthorblockA{
Department~of~Computer~Science\\
College~of~William~and~Mary\\
Williamsburg,~Virginia~23187--8795\\
Email:~mtufano@cs.wm.edu}
\and
\IEEEauthorblockN{Mat{\'i}as~Mart{\'i}nez}
\IEEEauthorblockA{
\td\\
University~of~Valenciennes\\
\td\\
Email:~\td}
\and
\IEEEauthorblockN{Martin~Monperrus}
\IEEEauthorblockA{
\td\\
University~of~Lille~and~INRIA\\
\td\\
Email:~martin.monperrus@univ-lille1.fr}
\and
\IEEEauthorblockN{Denys~Poshyvanyk}
\IEEEauthorblockA{
Department~of~Computer~Science\\
College~of~William~and~Mary\\
Williamsburg,~Virginia~23187--8795\\
Email:~denys@cs.wm.edu}
}
\end{comment}

==> scr/IEEE.preamble.tex <==
%\usepackage{booktabs,cite,comment,flushend,multirow,todonotes}
\usepackage{amsmath,amssymb,booktabs,cite,comment,flushend,listings,multirow,tikz,todonotes}
%\usepackage{graphicx,caption,subcaption}
\usetikzlibrary{arrows,calc,shapes}

% Text Encoding, Font Encoding, Microtypography
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{microtype}

\usepackage{tabularx}
\usepackage{hyperref}

% Widows and Orphans
\clubpenalty = 10000
\widowpenalty = 10000
\displaywidowpenalty = 10000

\DeclareGraphicsExtensions{.pdf,.png}
\graphicspath{{img/}}

\hyphenation{auto-encoder}

\newcommand{\denys}[1]{\todo[color=pink,inline]{#1}}
\newcommand{\dissertation}[1]{\iffalse{#1}\fi}
\newcommand{\ed}[1]{\textcolor{red}{#1}}
\newcommand{\seedtwo}[1]{\textcolor{black}{#1}}
\newcommand{\seedthr}[1]{\textcolor{black}{#1}}
\newcommand{\fm}{\textcolor{red}{FIXME}~}
\newcommand{\martin}[1]{\todo[color=blue!75,inline]{#1}}
\newcommand{\marty}[1]{\todo[inline]{#1}}
\newcommand{\matias}[1]{\todo[color=green!75,inline]{#1}}
\newcommand{\michele}[1]{\todo[color=yellow,inline]{#1}}
\newcommand{\reviewer}[1]{\todo[color=red,inline]{#1}}
\newcommand{\td}{\textcolor{red}{TODO}~}
\newcommand{\xx}{\textcolor{red}{XXX}~}

\makeatletter
\newcommand*{\defeqq}{\mathrel{\rlap{%
                     \raisebox{0.3ex}{$\m@th\cdot$$\m@th\cdot$}}%
                     \raisebox{-0.3ex}{$\m@th\cdot$$\m@th\cdot$}}%
                     =}
\makeatother

\lstset{language=Java,
%  numbers=left,
  showspaces=false,
  showtabs=false,
  breaklines=true,
  showstringspaces=false,
  breakatwhitespace=true,
  commentstyle=\color{green},
  keywordstyle=\color{blue},
  stringstyle=\color{red},
  basicstyle=\ttfamily\tiny,
  moredelim=[il][\textcolor{grey}]{$$},
  moredelim=[is][\textcolor{grey}]{\%\%}{\%\%}
}

==> scr/acmart.preamble.tex <==
%\usepackage{booktabs,cite,comment,flushend,multirow,todonotes}
\usepackage{booktabs,comment,flushend,listings,multirow,tikz,todonotes}
\usepackage{natbib}
\usepackage{graphicx,caption,subcaption}
\usetikzlibrary{arrows,calc,shapes}
%\begin{comment}
% Copyright
%\setcopyright{none}
%\setcopyright{acmcopyright}
%\setcopyright{acmlicensed}
\setcopyright{rightsretained}
%\setcopyright{usgov}
%\setcopyright{usgovmixed}
%\setcopyright{cagov}
%\setcopyright{cagovmixed}

% DOI
\acmDOI{10.475/123_4}

% ISBN
\acmISBN{123-4567-24-567/08/06}

%Conference
\acmConference[ESEC/FSE'17]{ACM SIGSOFT Symposium on the Foundations of Software Engineering}{September 2017}{Paderborn, Germany}
\acmYear{2017}
\copyrightyear{2017}

\acmPrice{15.00}
%\end{comment}
% Text Encoding, Font Encoding, Microtypography
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{microtype}

% Widows and Orphans
\clubpenalty = 10000
\widowpenalty = 10000
\displaywidowpenalty = 10000

\DeclareGraphicsExtensions{.pdf,.png}
\graphicspath{{img/}}

\newcommand{\denys}[1]{\todo[color=pink,inline]{#1}}
\newcommand{\dissertation}[1]{\iffalse{#1}\fi}
\newcommand{\ed}[1]{\textcolor{red}{#1}}
\newcommand{\fm}{\textcolor{red}{FIXME}~}
\newcommand{\martin}[1]{\todo[color=blue!75,inline]{#1}}
\newcommand{\marty}[1]{\todo[inline]{#1}}
\newcommand{\matias}[1]{\todo[color=green!75,inline]{#1}}
\newcommand{\michele}[1]{\todo[color=yellow,inline]{#1}}
\newcommand{\reviewer}[1]{\todo[color=red,inline]{#1}}
\newcommand{\td}{\textcolor{red}{TODO}~}
\newcommand{\xx}{\textcolor{red}{XXX}~}

\hyphenation{De-nys}

\lstset{language=Java,
%  numbers=left,
  showspaces=false,
  showtabs=false,
  breaklines=true,
  showstringspaces=false,
  breakatwhitespace=true,
  commentstyle=\color{green},
  keywordstyle=\color{blue},
  stringstyle=\color{red},
  basicstyle=\ttfamily\tiny,
  moredelim=[il][\textcolor{grey}]{$$},
  moredelim=[is][\textcolor{grey}]{\%\%}{\%\%}
}

==> scr/clones.tex <==
\begin{table}[t]
%\scriptsize
\caption{Number~of~Ingredients~Attempted~\td}
\label{tab:clones}
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
Scope						& Random	& Similar Executable	& Similar Type\\
\midrule
\begin{comment}
Local	& \td		& \td			& \td\\
Package	& \td		& \td			& \td\\
Global	& \td		& \td			& \td\\
\end{comment}
\multirow{4}{*}{Local}		& $y_{111}$	& $y_{121}$		& $y_{131}$\\
							& $y_{112}$	& $y_{122}$		& $y_{132}$\\
							& \dots		& \dots			& \dots\\
							& $y_{11m}$	& $y_{12m}$		& $y_{13m}$\\
\midrule
\multirow{4}{*}{Package}	& $y_{211}$	& $y_{221}$		& $y_{231}$\\
							& $y_{212}$	& $y_{222}$		& $y_{232}$\\
                        	& \dots		& \dots			& \dots\\
                        	& $y_{21m}$	& $y_{22m}$		& $y_{23m}$\\
\midrule
\multirow{4}{*}{Global}		& $y_{311}$	& $y_{321}$		& $y_{331}$\\
							& $y_{312}$	& $y_{322}$		& $y_{332}$\\
                        	& \dots		& \dots			& \dots\\
                        	& $y_{31m}$	& $y_{32m}$		& $y_{33m}$\\
\bottomrule
\end{tabular}
\end{table}

==> scr/embeddings.tex <==
\begin{table}[t]
%\scriptsize
\caption{Number~of~Ingredients~Rejected~\td}
\label{tab:embeddings}
\centering
\begin{tabular}{@{}lcc@{}}
\toprule
Scope						& Default	& Embeddings\\
\midrule
\multirow{4}{*}{Local}		& $y_{111}$				& $y_{121}$\\
							& $y_{112}$				& $y_{122}$\\
							& \dots					& \dots\\
							& $y_{11p}$				& $y_{12p}$\\
\midrule
\multirow{4}{*}{Package}	& $y_{211}$				& $y_{221}$\\
							& $y_{212}$				& $y_{222}$\\
                        	& \dots					& \dots\\
                        	& $y_{21p}$				& $y_{22p}$\\
\midrule
\multirow{4}{*}{Global}		& $y_{311}$				& $y_{321}$\\
							& $y_{312}$				& $y_{322}$\\
                        	& \dots					& \dots\\
                        	& $y_{31p}$				& $y_{32p}$\\
\bottomrule
\end{tabular}
\end{table}

==> sec/scratch.tex <==
\section{Scratch}

\marty{THINKING: Line-level analysis involves the data flow to *.distances.csv. Token-level analysis involves the data flow to clustering.csv.}

\subsection{Input~data}
Defects4J has five projects and each project has some number of bugs.
WLOG assume we are analyzing one bug for one project, e.g., Chart-1.

\subsection{Our approach is a pipeline with three phases}
Our approach will be organized in a pipeline architecture.
Our pipeline will have three phases: recognition, learning, and repair.
The recognition phase will precede the learning phase which will precede the repair phase.
% * <matomartinez@gmail.com> 2016-09-21T08:34:59.113Z:
%
% 3 phrase: are the three phases executed for each bug to repair?
% Or: phases Recognition and Learning are executed ones (given a code corpus) , and then, for each bug, Repair phase is executed?
%
% ^.
\begin{itemize}
\item \textbf{Recognition~phase.} The goal of the language recognition phase will be to consume in situ source code and produce training data.
\item \textbf{Learning~phase.} The goal of the machine learning phase will be to consume training data and produce machines for automatically representing source code at any level of granularity from lexical elements to compilation units. These machines will be reified as tensors.
% * <martin.monperrus@univ-lille1.fr> 2016-09-29T15:44:26.515Z:
%
% > reified as tensors
%
% not sure the average SE reader can understand
%
% ^.
% * <martin.monperrus@univ-lille1.fr> 2016-09-29T15:43:59.507Z:
%
% > machines
%
% machines? potentially confusing terminologu
%
% ^.
\item \textbf{Repair~phase.} The goal of the program repair phase will be to consume in situ source code and use the language recognizer and trained machines to produce a patch.
\end{itemize}
This pipeline takes us from in situ source code to a patch, but we will only be evaluating a slice of the pipeline, viz. number of ingredients attempted before breaking the fix ingredient search loop as well as quality attributes to evaluate our learning-based approach.

\subsection{Stages~of~the~recognition~phase}
\begin{enumerate}
\item \textbf{Parse.} Input: src. Output: ASTs. The first stage of recognition consumes in situ source code and produces ASTs. We will use Spoon to build the ASTs.
\item \textbf{Synthesize~corpora.} Input: ASTs. Output: corpora. The second stage of recognition visits the ASTs and produces corpora at different levels of granularity. We will produce corpora at three levels of granularity: file, class, and method. The corpus at each level of granularity will constitute two files, i.e., files.\{key,src\}, classes.\{key,src\}, and methods.\{key,src\}. Each line in a .key file will contain a unique ID for a programming construct at the corresponding level of granularity. Each line in a .src file will contain the corresponding source code (splayed on the line). We’ve already touched on post-conditions for these files in the Astor email thread. However, there is one decision that we need to make for classes. Do we simply consider top-level classes? Or do we break out (static and non-static) nested classes? Recall that statements in similar classes are going to be attempted before statements in dissimilar classes. My thought is we only measure similarity between top-level classes. Likewise, for executables, we only consider top-level executables. (I think methods can contain anonymous executables.)
% * <martin.monperrus@univ-lille1.fr> 2016-09-29T15:45:35.260Z:
%
% > Do we simply consider top-level classes? 
%
% I'd say, yes, it(s simpler. IMHO the impact of sophistication will be small
%
% ^.
\item \textbf{Normalize corpora.} Input: corpora. Output: normalized corpora. I think the only normalization worth considering is how literal values are handled. There are six different literal types: BooleanLiteral, CharacterLiteral, FloatingPointLiteral, IntegerLiteral, NullLiteral, and StringLiteral. Since we will be using a fast algorithm for learning embeddings and considering the modest size of our corpora, vocabulary sizes will not be an issue. We probably don’t even need to normalize the corpora so this is another decision we need to make. Do we map literal values to their respective type? If so, normalize all types? Just ints and floats? Just strings? Just numbers and strings?
% * <martin.monperrus@univ-lille1.fr> 2016-09-29T15:46:41.437Z:
%
% > We probably don’t even need to normalize the corpora so this is another decision we need to make. 
%
% I would first try without normalization
%
% ^.
\end{enumerate}

\subsection{Stages~of~the~learning~phase}
\begin{enumerate}
\item \textbf{word2vec.} Input: files.src. Output: dictionary.txt. word2vec was designed for inducing word embeddings from a massive corpus. We won’t be working with massive corpora for this project but we’ll use word2vec rather than a recurrent net because training is much faster and the embeddings are only intended to serve as rough priors for the recursive autoencoders. dictionary.txt will be the word2vec output which will contain the mapping from lexical elements to embeddings.
% * <martin.monperrus@univ-lille1.fr> 2016-09-29T15:47:40.264Z:
%
% > word2vec
%
% what is this?
%
% ^.
\item \textbf{k-means.} Input: dictionary.txt. Output: classes.txt. Runs k-means on the embeddings to categorize lexical elements. k will be equal to the square root of the vocabulary size. Of course, we have the option of using another clustering algorithm given a compelling reason. The purpose of categorizing embeddings is described below.
% * <martin.monperrus@univ-lille1.fr> 2016-09-29T15:48:09.797Z:
%
% > embeddings
%
% not clear. is it a numerical vector? what range? which distance metric used? (if already answered, a ref is OK)
%
% ^.
\item \textbf{RAE.} Input: files.src and dictionary.txt. Output: encoder.mat and similarities.txt. The autoencoders will be trained on files.src which is the file-level corpus. Once the encoders are trained we can compute an embedding for anything from a lexical element to a compilation unit. Then we use the encoders to encode each method and every class so we can cache the method- and class-level similarities in similarities.txt.
\end{enumerate}

\subsection{Stages~of~the~repair~phase}
\begin{enumerate}
\item \textbf{Fault~localization.} Input: src and regression test cases. Output: list of suspicious statements. Fault localization consumes source code and a test suite and computes a list of suspicious statements.
\item \textbf{Repair~operator.} Input: random variate. Output: repair operator. JGenProg randomly selects one of four repair operators: InsertAfterOp, Insert BeforeOp, RemoveOp, and ReplaceOp.
\item \textbf{Fix~ingredient.} Input: list of suspicious statements and repair operator. Output: evaluation metrics. Suspicious statements will be prioritized according to their suspicious values (in [0, 1]) from most suspicious to least suspicious. Once a suspicious statement is selected from the list of suspicious statements, the selected statement is modified according to a repair operator. If the repair operator is RemoveOp then our strategy will not come into play; our strategy will come into play when the repair operator inserts or replaces statements. WLOG assume the clone granularity is set to class. First, we query the class of the selected statement. Then we query a list of classes in scope (which will be set to either local, package, or global) sorted by similarity (from similarities.txt). Then we loop through the sorted list of classes extracting their statements in order. (There’s an opportunity to apply more filtering here but v1.0 will be basic.) Finally we use this fix space representation and start computing our evaluation metrics. (Note that ReplaceOp will still have the same type check.)
% * <matomartinez@gmail.com> 2016-09-21T08:38:26.588Z:
%
% Minor comment: 
% As the selection of the operator is in a previous step, I would put a new step for selecting an statement from the suspicious list. 
% or: One step for selecting both suspicious and operator.
%
% ^.
\item \textbf{Embeddings.} We are also going to look at how using word embeddings to transform otherwise semantically incorrect ingredients affects the evaluation metrics. When the VariableResolver analyzes fitInPlace, the first thing it does is query the variable context of the modification point. Then it collects the ingredient’s variable accesses, and computes whether the <name, type> of each variable access corresponds to a <name, type> in the modification point’s variable context. If there isn’t a match then the ingredient is discarded and the procedure attempts the new candidate ingredient. The update we’ll make to the matching engine (VariableResolver.matchVariable) is the flag (boolean matchName) will now perform the following check. We’ll take all “unbound” names in the context and sort them according to the proximity of their embeddings with the embedding of the variable access. If the closest embedding is also in the same class (per classes.txt in the learning phase) then we’ll replace the variable access in the ingredient before attempting it. If there is more than one variable access that is out of context then we’ll implement simple bookkeeping to transform multiple variables accesses.
% * <matomartinez@gmail.com> 2016-09-21T08:44:52.874Z:
% 
% Minor: "same class" ==> 
% do you mean: a) same cluster , or 
% b) same Type of the variable access (i.e., int, string)? 
% I imagine is option a)
% 
% ^.
\end{enumerate}

\subsection{Miscellaneous}

\marty{THINKING: The analysis phase of the compiler concerns decomposition. The synthesis phase concerns \xx}

==> sec/unused-text.tex <==


BELOW: old text from III.C

For example, running spectrum-based fault localization~\cite{Abreu:2006} on Math-63 yields eight statements with suspicious values greater than 0.1~%


{Once  DeepRepair creates the list of ingredients from similar executables, it proceeds by taking in order ingredients from that list and to create candidate repairs for a randomly selected operator. 
For each ingredient, DeepRepair checks if all variables from the ingredient are in scope at the modification point. If it is the case, that means the ingredients can be used "as is" as patch ingredient, without applying any transformation. Therefore, DeepLearning creates the candidate patch , applies it to the buggy program and then evaluates it using the buggy program's test suite.
Otherwise, when the ingredient has at least one variable that is not in the scope at the modification point, DeepRepairs aims at refining the ingredient to create a candidate patch.
For that, DeepRepair applies a strategy to replace them by variables in scope: TODO: continue with the existing explanation from paragraph: "To find a patch".
}

In this work, we consider two levels of granularities: Executables (methods) and Types. In the remain of this section, we describe DeepRepair using the executable level.
DeepRepair uses the cached, executable-level similarity list to sort methods in the codebase {\it{according to the similitude with the executable that contains the modification points}}.~%
Here, DeepRepair also takes in account the ingredient scope as explained in Section\ref{}, for instance, if the ingredient scope is "Local",  the list only includes methods from the same  file.
Then, DeepRepair extracts the statements (i.e., ``ingredients'') from each method in turn and enqueue them in a first-in first-out queue.
}

When we evolve the program, in a generation, we randomly select a repair operator (e.g., InsertAfterOp) and poll an ingredient.~%
The operator and the ingredient form a {modification~instance}.~%
We test whether all of the variable accesses in the modification instance are in scope at the modification point, and mutate the program accordingly \ed{to generate a candidate patch}.~%
If the modification instance has variables accesses that are either out of scope or the modification instance has already been applied, then we poll an \ed{a new} ingredient to attempt a new modification instance.~%

